EMOPortraits: Emotion-enhanced Multimodal One-shot Head Avatars

Head avatars animated by visual signals have gained popularity, particularly in cross-driving synthesis where the driver differs from the animated character, a challenging but highly practical approach. The recently presented MegaPortraits model has demonstrated state-of-the-art results in this domain. We conduct a deep examination and evaluation of this model, with a particular focus on its latent space for facial expression descriptors, and uncover several limitations with its ability to express intense face motions. To address these limitations, we propose substantial changes in both training pipeline and model architecture, to introduce our EMOPortraits model, where we: Enhance the model's capability to faithfully support intense, asymmetric face expressions, setting a new state-of-the-art result in the emotion transfer task, surpassing previous methods in both metrics and quality. Incorporate speech-driven mode to our model, achieving top-tier performance in audio-driven facial animation, making it possible to drive source identity through diverse modalities, including visual signal, audio, or a blend of both. We propose a novel multi-view video dataset featuring a wide range of intense and asymmetric facial expressions, filling the gap with absence of such data in existing datasets.

==> figs/can_vol_vis.tex <==
\begin{figure}[H]
    \centering
    % \setlength{\wid}{0.09\textwidth}
    % \includegraphics[width=\linewidth]{}
    \includegraphics[width=1\linewidth]{figs/vis_can_vol.png}
    \caption{Canonical volume visualisation}
    \label{fig:curr_dataset_vision}
\end{figure}
\vspace{-8pt}


==> figs/datasets_stat_comp.tex <==
\begin{figure}[H]
    \centering
    % \setlength{\wid}{0.09\textwidth}
    % \includegraphics[width=\linewidth]{}
    \includegraphics[width=1\linewidth]{figs/dens2.png}
    \caption{Asymmetry score distribution across datasets}
    \label{fig:datasets_stat}
\end{figure}
\vspace{-12pt}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

